Segment Any Cell: A SAM-based Auto-prompting Fine-tuning Framework for Nuclei Segmentation

In the rapidly evolving field of AI research, foundational models like BERT and GPT have significantly advanced language and vision tasks. The advent of pretrain-prompting models such as ChatGPT and Segmentation Anything Model (SAM) has further revolutionized image segmentation. However, their applications in specialized areas, particularly in nuclei segmentation within medical imaging, reveal a key challenge: the generation of high-quality, informative prompts is as crucial as applying state-of-the-art (SOTA) fine-tuning techniques on foundation models. To address this, we introduce Segment Any Cell (SAC), an innovative framework that enhances SAM specifically for nuclei segmentation. SAC integrates a Low-Rank Adaptation (LoRA) within the attention layer of the Transformer to improve the fine-tuning process, outperforming existing SOTA methods. It also introduces an innovative auto-prompt generator that produces effective prompts to guide segmentation, a critical factor in handling the complexities of nuclei segmentation in biomedical imaging. Our extensive experiments demonstrate the superiority of SAC in nuclei segmentation tasks, proving its effectiveness as a tool for pathologists and researchers. Our contributions include a novel prompt generation strategy, automated adaptability for diverse segmentation tasks, the innovative application of Low-Rank Attention Adaptation in SAM, and a versatile framework for semantic segmentation challenges.

==> sec/5_limitations.tex <==
\section{Discussion}
\label{sec:limit}
Our proposed SAC is the first to introduce an auto-prompting method for nuclei segmentation. Diverging from other studies that focus on designing fine-tuning models, our method seeks to enhance prompt quality by adopting a prompt generator. This generator automatically creates high-quality prompts for given medical images,  improving not only the segmentation performance but also efficiency. 
Extensive experiments show that our proposed SAC has achieved promising results in the automatic generation of point prompts for cell nucleus segmentation tasks. Given the versatility of our method, it can be easily adapted to other tasks that may require different formats of prompts. For instance, if a task requires ``box prompt``, our method can be modified to include the maximum bounding box of the object mask as the prompt label. Furthermore, to enhance cell segmentation performance, we plan to gather more cell segmentation data and train a cell nucleus segmentation foundation model as a replacement for SAM.
% Extensive experiments demonstrate that our proposed SAC has obtained promising results for the automatic generation of point prompts in cell nucleus segmentation tasks. Considering the extendability of our method on other tasks that might require different formats of prompts, our method can be easily adapted to them as well. For example, if the task requires ``box prompts``, our method can be modified by incorporating maximum bounding box of the object mask as the prompt label. 
% Moreover, for further improvement of the cell segmentation performance, we plan to collect more cell segmentation data and train a cell nucleus segmentation foundation model in place of SAM. 

% Despite the promising results obtained from our proposed SAC, there remains room for improvement. Firstly, our current SAC framework primarily supports the automatic generation of point prompts, which are adequate for cell nucleus segmentation tasks. However, for application in other tasks, different types of prompt generation may be necessary. For instance, for tasks requiring 'box prompts,' our training approach for the prompt generator can incorporate the use of the maximum bounding box of the object mask as the prompt label. 
% % 第一点要表现我们的方法在细胞分割上 生成点的prompt的方式已经结果非常好了,要是将这个idea应用到其他的领域,可能需要生成其他种类的prompt,比如,如果需要'box prompt',我们在训练prompt generator的时候可以使用待分割物体mask的最大边界组成的box作为prompt label.
% Moreover, while our method is efficient in quickly training for different types of cell segmentation tasks, enhancing the universality of our model remains a priority. To achieve this, we plan to collect a diverse range of data encompassing various cell types. This comprehensive dataset will then be used to train a unified, robust model for cell segmentation. Such an approach not only broadens the applicability of our SAC model but also ensures its adaptability to a wider spectrum of segmentation challenges in cellular biology. 
% 第二点改一下 主要是说我们在未来要收集更多的细胞分割数据,训练一个基于细胞核分割的foundation model替换掉原有的SAM,可能会获得更好的结果







==> sec/N_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
